Diff3DS: Generating View-Consistent 3D Sketch via Differentiable Curve Rendering

3D sketches are widely used for visually representing the 3D shape and structure of objects or scenes. However, the creation of 3D sketch often requires users to possess professional artistic skills. Existing research efforts primarily focus on enhancing the ability of interactive sketch generation in 3D virtual systems. In this work, we propose Diff3DS, a novel differentiable rendering framework for generating view-consistent 3D sketch by optimizing 3D parametric curves under various supervisions. Specifically, we perform perspective projection to render the 3D rational B\'ezier curves into 2D curves, which are subsequently converted to a 2D raster image via our customized differentiable rasterizer. Our framework bridges the domains of 3D sketch and raster image, achieving end-toend optimization of 3D sketch through gradients computed in the 2D image domain. Our Diff3DS can enable a series of novel 3D sketch generation tasks, including textto-3D sketch and image-to-3D sketch, supported by the popular distillation-based supervision, such as Score Distillation Sampling (SDS). Extensive experiments have yielded promising results and demonstrated the potential of our framework. Project page is at https://yiboz2001.github.io/Diff3DS/.

==> figure/analysis1_2.tex <==
\begin{figure}[h]
\vspace{-0.25cm}
\centering
\begin{minipage}{0.443\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/media/analysis_cfg_fix.pdf}
    \vspace{-0.5cm}
    \caption{Effect of CFG weight.}
    \label{fig:ablation_cfg}
\end{minipage}
\hfill
\begin{minipage}{0.537\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/media/analysis_backbone_fix.pdf}
    \vspace{-0.5cm}
    \caption{Effect of the impact of pre-trained models.}
    \label{fig:analysis_backbone}
\end{minipage}
\vspace{-0.6cm}
\end{figure}


==> figure/analysis_backbone.tex <==
\begin{figure}[t!]
    \includegraphics[width=1 \textwidth]{figure/media/analysis_backbone.pdf}
    \caption{\textbf{Analysis of the impact of different pre-trained model}}
    \label{fig:analysis_backbone}
\end{figure}

==> figure/analysis_cfg.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{figure/media/analysis_cfg.pdf}
    \caption{\textbf{Analysis of the impact of CFG weight}}
    \label{fig:ablation_cfg}
\end{figure}

==> figure/projection.tex <==
\begin{wrapfigure}[]{r}{0.30\textwidth}
    % \vspace{-1cm}
    \centering
    \includegraphics[width=0.30\textwidth]{figure/media/projection.pdf}
    \vspace{-0.6cm}
    \caption{Pseudo ground truth}
    \label{fig:projection}
    % \vspace{0.3cm}
\end{wrapfigure}


==> figure/train_process.tex <==
% \begin{wrapfigure}[5]{r}{0.50\textwidth}
%     \vspace{-0.70cm}
%     \includegraphics[width=0.50\textwidth]{figure/media/train_process.pdf}
%     \vspace{-0.8cm}
%     \caption{Illustration of the optimization process.}
%     \label{fig:train_process}
%     % \vspace{-0.5cm}
% \end{wrapfigure}


\begin{figure}[h]
  \centering
  \vspace{-0.28cm}
  \includegraphics[width=1\textwidth]{figure/media/train_process2.pdf}
  \vspace{-0.6cm}
  \caption{Illustration of the optimization process.}
  \vspace{-0.5cm}
  \label{fig:train_process}
\end{figure}





==> sec/7_addational_pages.tex <==
\clearpage
\input{figure/More Text Generated Results}
\clearpage
\input{figure/More Image Generated Results}
\clearpage


==> table/compare_1.tex <==
\begin{table}[t]
    \centering
    \caption{Quantitative results of the text-to-3D sketch task. }
    \vspace{-0.2cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    
        \centering
        \begin{tabular}{l|ccc}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}*{\textbf{Method}}} 
        & \multicolumn{2}{c}{ \textbf{CLIP-Score$\rm ^{T}$} $\uparrow$ }     
        &  \multicolumn{1}{c}{
            \multirow{2}*{\textbf{BLIP-Score} $\uparrow$}
        } 
        \\
        
        \multicolumn{1}{c|}{~}                              
        & ViT B/16 & ViT B/32 \\ \midrule
        
        % DiffSketcher  \cite{xing2023diffsketcher}
        % & \cellcolor{lightgray} 33.64 & \cellcolor{lightgray} 33.98 \\ \midrule 
        
        DreamGaussian \cite{tang2023dreamgaussian}
        & 0.2561  & 0.2453 & 0.4990 \\
        
        MVDream \cite{shi2023mvdream}
        & 0.2763  & 0.2653 & 0.4949 \\ 
        
        Diff3DS (Ours) 
        & \textbf{0.3046} & \textbf{0.3034} & \textbf{0.5038}\\ \bottomrule
        
        \end{tabular}%
    
    \label{tab:compare_to_text_3d_baseline}    
\end{table}


==> table/compare_2.tex <==
% \begin{table}[t]
%     \centering   
%     \caption{Quantitative results of the image-to-3D sketch task.}
%     \label{tab:compare_to_img_3d_baseline}
%     \vspace{-0.2cm}
%     \newcommand{\tabincell}[2]{
%         \begin{tabular}{@{}#1@{}}#2\end{tabular}
%     }
%     \centering

%     \begin{tabular}{l|ccc}
%     \toprule
    
%     \multicolumn{1}{c|}{
%         \multirow{2}*{\textbf{Method}}
%     } 
%     & \multicolumn{2}{c}{ 
%         \textbf{CLIP-Score$\rm ^{I}$} $\uparrow$   
%     }
%     &  \multicolumn{1}{c}{
%         \multirow{2}*{\textbf{LPIPS} $\downarrow$}
%     } 
%     \\
    
%     \multicolumn{1}{c|}{~}                              
%     & ViT B/16 & ViT B/32 \\ \midrule
    
%     % CLIPasso \cite{vinker2022clipasso} 
%     % & \cellcolor{lightgray} 83.79
%     % & \cellcolor{lightgray} 82.72
%     % \\ \midrule
    
%     NEF \cite{ye2023nef}
%     & 66.12
%     & 66.05
%     & 0.399
%     \\ 

%     3Doodle \cite{choi20243doodle}
%     & 67.34
%     & 67.46
%     & \textbf{0.256}
%     \\ 
    
%     Diff3DS (Ours)  
%     & \textbf{67.68}
%     & \textbf{68.46}
%     & 0.264
%     \\ \bottomrule
%     \end{tabular}%
% \end{table}


\begin{table}[t]
    \centering     
    \caption{Quantitative results of the image-to-3D sketch task.}

        \label{tab:compare_to_img_3d_baseline}
        \vspace{-0.2cm}
        \newcommand{\tabincell}[2]{
            \begin{tabular}{@{}#1@{}}#2\end{tabular}
        }
        \centering
    
        \begin{tabular}{l|ccc}
        \toprule
        
        \multicolumn{1}{c|}{
            \multirow{2}*{\textbf{Method}}
        } 
        & \multicolumn{2}{c}{ 
            \textbf{CLIP-Score$\rm ^{I}$} $\uparrow$   
        }
        &  \multicolumn{1}{c}{
            \multirow{2}*{\textbf{LPIPS} $\downarrow$}
        } 
        \\
        
        \multicolumn{1}{c|}{~}                              
        & ViT B/16 & ViT B/32 \\ \midrule
        
        % CLIPasso \cite{vinker2022clipasso} 
        % & \cellcolor{lightgray} 83.79
        % & \cellcolor{lightgray} 82.72
        % \\ \midrule
        
        NEF \cite{ye2023nef}
        & 0.6612
        & 0.6605
        & 0.3997
        \\ 
    
        3Doodle \cite{choi20243doodle}
        & 0.6734
        & 0.6746
        & \textbf{0.2567}
        \\ 
        
        Diff3DS (Ours)  
        & \textbf{0.6768}
        & \textbf{0.6846}
        & 0.2647
        \\ \bottomrule
        \end{tabular}%
    
    % \end{minipage}
\end{table}


==> table/compare_to_img_3d_baseline.tex <==
\begin{table}[t] 
\caption{\textbf{Quantitative results of the image-to-3D sketch task}}
\label{tab:compare_to_img_3d_baseline}

\centering

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc}
\toprule

\multicolumn{1}{c|}{\multirow{2}*{\textbf{Method}}} 
& \multicolumn{2}{c}{ \textbf{CLIP-Score$\rm ^{I}$} $\uparrow$ }     \\

\multicolumn{1}{c|}{~}                              
& ViT B/16 & ViT B/32 \\ \midrule

CLIPasso \cite{vinker2022clipasso} 
& \cellcolor{lightgray} 82.26 
& \cellcolor{lightgray} xxxx
\\ \midrule

NEF \cite{ye2023nef}
& xxxx
& xxxx
\\ 

Our  
& 78.03 
& xxxx 
\\ \bottomrule
\end{tabular}%
}
\end{table}


==> table/compare_to_text_3d_baseline.tex <==
\begin{table}[t]
\caption{\textbf{Quantitative results of the text-to-3D sketch task}}
\label{tab:compare_to_text_3d_baseline}

\centering

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc}
\toprule

\multicolumn{1}{c|}{\multirow{2}*{\textbf{Method}}} 
& \multicolumn{2}{c}{ \textbf{CLIP-Score$\rm ^{T}$} $\uparrow$ }     \\

\multicolumn{1}{c|}{~}                              
& ViT B/16 & ViT B/32 \\ \midrule
  

DiffSketcher  \cite{xing2023diffsketcher}
& \cellcolor{lightgray} 33.64 & \cellcolor{lightgray} 33.98 \\ \midrule 

DreamGaussian \cite{tang2023dreamgaussian}
& 26.25  & 25.12 \\

MVDream \cite{shi2023mvdream}
& 28.39  & 27.08 \\ 

Our 
& \textbf{30.35} & \textbf{30.00} \\ \bottomrule

\end{tabular}%
}

\end{table}
















% \begin{table}[t!]
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|cc}
% \toprule
% \textbf{Method} &
%   \textbf{CLIP-Score} $\uparrow$ &
%   \textbf{CLIP-R-Precision(\%)} $\uparrow$
%   \\ \midrule
  

% DiffSketcher  \cite{xing2023diffsketcher}
% & \cellcolor{lightgray} 33.98 &  \cellcolor{lightgray} 94.2 \\ \midrule 
% DreamGaussian \cite{tang2023dreamgaussian}
% & 25.12          & \textbf{71.4} \\
% MVDream \cite{shi2023mvdream}
% & 26.48          & 62.8 \\ 
% Our 
% & \textbf{30.71}   & \textbf{71.4} \\ \bottomrule
% \end{tabular}%
% }

% \caption{\textbf{Quantitative results of the text-to-3D curves task}}
% \vspace{-6mm}
% \label{tab:compare_to_text_3d_baseline}
% \end{table}

